Single Channel Audio Source Separation using Convolutional Denoising Autoencoders

Deep learning techniques have been used recently to tackle the audio source separation problem. In this work, we propose to use deep fully convolutional denoising autoencoders (CDAEs) for monaural audio source separation. We use as many CDAEs as the number of sources to be separated from the mixed signal. Each CDAE is trained to separate one source and treats the other sources as background noise. The main idea is to allow each CDAE to learn suitable spectral-temporal filters and features to its corresponding source. Our experimental results show that CDAEs perform source separation slightly better than the deep feedforward neural networks (FNNs) even with fewer parameters than FNNs.

==> def_bold.tex <==
%       def,bold.tex
%       Bold math symbols

%       use amsbsy and \pmb for "poor man's bold" for greek subscripts
%       lower case greek are "symbols"  (p. 53)

\providecommand{\myboldg}[1]    {\mbox{\boldmath $#1$}}         % lower greek
\providecommand{\myboldG}       {\myboldg}                      % upper greek
%\providecommand{\mybolda}[1]   {\ensuremath{\mathbf{#1}}}      % lower alpha
%\providecommand{\mybolda}[1]   {\ensuremath{\mathit{\mathbf{#1}}}}     % lower alpha
\providecommand{\mybolda}       {\myboldg}                      % lower alpha
\providecommand{\myboldA}       {\mybolda}                      % upper alpha
\providecommand{\myboldn}       {\mybolda}                      % numbers

% small bold for subscripts and superscripts
\providecommand{\boldscript}[1] {\mbox{\boldmath\scriptsize$#1$}}

\providecommand{\Bzero} {\myboldn{0}}
\providecommand{\Bone}  {\myboldn{1}}
\providecommand{\bZero} {\myboldn{0}}

\providecommand{\Ba}{\mybolda{a}}
\providecommand{\Bb}{\mybolda{b}}
\providecommand{\Bc}{\mybolda{c}}
\providecommand{\Bd}{\mybolda{d}}
\providecommand{\Be}{\mybolda{e}}
\providecommand{\Bf}{\mybolda{f}}
\providecommand{\Bg}{\mybolda{g}}
\providecommand{\Bh}{\mybolda{h}}
\providecommand{\Bi}{\mybolda{i}}
\providecommand{\Bj}{\mybolda{j}}
\providecommand{\Bk}{\mybolda{k}}
\providecommand{\Bl}{\mybolda{l}}
\providecommand{\Bm}{\mybolda{m}}
\providecommand{\Bn}{\mybolda{n}}
\providecommand{\Bo}{\mybolda{o}}
\providecommand{\Bp}{\mybolda{p}}
\providecommand{\Bq}{\mybolda{q}}
\providecommand{\Br}{\mybolda{r}}
\providecommand{\Bs}{\mybolda{s}}
\providecommand{\Bt}{\mybolda{t}}
\providecommand{\Bu}{\mybolda{u}}
\providecommand{\Bv}{\mybolda{v}}
\providecommand{\Bw}{\mybolda{w}}
\providecommand{\Bx}{\mybolda{x}}
\providecommand{\By}{\mybolda{y}}
\providecommand{\Bz}{\mybolda{z}}

\providecommand{\bA}{\myboldA{A}}
\providecommand{\bB}{\myboldA{B}}
\providecommand{\bC}{\myboldA{C}}
\providecommand{\bD}{\myboldA{D}}
\providecommand{\bE}{\myboldA{E}}
\providecommand{\bF}{\myboldA{F}}
\providecommand{\bG}{\myboldA{G}}
\providecommand{\bH}{\myboldA{H}}
\providecommand{\bI}{\myboldA{I}}
\providecommand{\bJ}{\myboldA{J}}
\providecommand{\bK}{\myboldA{K}}
\providecommand{\bL}{\myboldA{L}}
\providecommand{\bM}{\myboldA{M}}
\providecommand{\bN}{\myboldA{N}}
\providecommand{\bO}{\myboldA{O}}
\providecommand{\bP}{\myboldA{P}}
\providecommand{\bQ}{\myboldA{Q}}
\providecommand{\bR}{\myboldA{R}}
\providecommand{\bS}{\myboldA{S}}
\providecommand{\bT}{\myboldA{T}}
\providecommand{\bU}{\myboldA{U}}
\providecommand{\bV}{\myboldA{V}}
\providecommand{\bW}{\myboldA{W}}
\providecommand{\bX}{\myboldA{X}}
\providecommand{\bY}{\myboldA{Y}}
\providecommand{\bZ}{\myboldA{Z}}

\providecommand{\Balpha}        {\myboldg{\alpha}}
\providecommand{\Bbeta}         {\myboldg{\beta}}
\providecommand{\Bchi}          {\myboldg{\chi}}
\providecommand{\Bdelta}        {\myboldg{\delta}}
\providecommand{\Beps}          {\myboldg{\epsilon}}
\providecommand{\Bveps}         {\myboldg{\varepsilon}}
\providecommand{\Bgamma}        {\myboldg{\gamma}}
\providecommand{\Blambda}       {\myboldg{\lambda}}
\providecommand{\Bmu}           {\myboldg{\mu}}
\providecommand{\Bphi}          {\myboldg{\phi}}
\providecommand{\Bpsi}          {\myboldg{\psi}}
\providecommand{\Btau}          {\myboldg{\tau}}
\providecommand{\Btheta}        {\myboldg{\theta}}
\providecommand{\Brho}          {\myboldg{\rho}}
\providecommand{\Bzeta}         {\myboldg{\zeta}}
\providecommand{\Bxi}           {\myboldg{\xi}}
\providecommand{\Bsigma}        {\myboldg{\sigma}}

\providecommand{\bGam}          {\myboldG{\Gamma}}
\providecommand{\bLam}          {\myboldG{\Lambda}}
\providecommand{\bOm}           {\myboldG{\Omega}}
\providecommand{\bPi}           {\myboldG{\Pi}}
\providecommand{\bPhi}          {\myboldG{\Phi}}
\providecommand{\bPsi}          {\myboldG{\Psi}}
\providecommand{\bSig}          {\myboldG{\Sigma}}
\providecommand{\bSigma}        {\myboldG{\Sigma}}
\providecommand{\bTheta}        {\myboldG{\Theta}}


\providecommand{\cR}            {\ensuremath{\cal R}}
\providecommand{\cS}            {\ensuremath{\cal S}}
\providecommand{\cM}            {\ensuremath{\cal M}}

